Minions: Cost-efficient Collaboration Between On-device and Cloud Language Models

We investigate an emerging setup in which a small, on-device language model (LM) with access to local data communicates with a frontier, cloud-hosted LM to solve real-world tasks involving financial, medical, and scientific reasoning over long documents. Can a local-remote collaboration reduce cloud inference costs while preserving quality? First, we consider a naive collaboration protocol where the local and remote models simply chat back and forth. Because only the local model reads the full context, this protocol achieves a 30.4x reduction in remote costs, but recovers only 87% of the performance of the frontier model. We identify two key limitations of this protocol: the local model struggles to (1) follow the remote model's multi-step instructions and (2) reason over long contexts. Motivated by these observations, we study an extension of this protocol, coined MinionS, in which the remote model decomposes the task into easier subtasks over shorter chunks of the document, that are executed locally in parallel. MinionS reduces costs by 5.7x on average while recovering 97.9% of the performance of the remote model alone. Our analysis reveals several key design choices that influence the trade-off between cost and performance in local-remote systems.

==> figures/lm-bottleneck/local-lm-bottleneck.tex <==


\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/lm-bottleneck/plot.pdf}
    \caption{\textbf{Communication efficiency of \system when utilizing different local LM's.} x-axis is the total number of token sent up to the remote model. We observe that larger local models (7-8B parameters) are more token efficient than smaller LMs.
    }
    \label{fig:lm-bottleneck}
  \end{figure}




==> figures/model-longitudinal/model-longitudinal.tex <==



\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{figures/model-longitudinal/plot.pdf}
    \caption{\textbf{Edge-remote quality over time.} The x-axis represents the date of release.
}
    \label{fig:model-longitudinal}
  \end{figure}




==> figures/scaling-samples-latency/scaling-samples.tex <==



\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/scaling-samples/plot.png}
    \caption{\textbf{Exploring the trade-off between cost and quality with sampling at the edge.} The x-axis represents the number of tokens processed by the \textit{local model}, while the y-axis shows the accuracy achieved. Foreground dots connected by a line highlight the trend in accuracy improvement as the number samples (and remote tokens processed). The vertical  lines denote the point at which batched, parallel sampling is no longer compute efficient.}
    \label{fig:scaling-samples}
\end{figure}


==> sections/archive/introduction_jan_22.tex <==
\section{Introduction}
\label{sec:intro}
Today's frontier Language Models (LMs) can program across repositories and make complex decisions in financial, legal, and medical domains. However, accessing these models is expensive: processing a standard million-token code repository with OpenAI's o1 API costs $>\$15$ per query. 
% 
At the same time, smaller LMs (1-7B parameters) are rapidly improving and can now run on personal computers (ollama, llama.cpp) and smartphones (OpenELM, PhoneLM)  (\textit{e.g.} an \textcolor{red}{XX} model can process \textcolor{red}{XX} tokens per second on a phone). But these small LMs are not participating in challenging reasoning tasks, leaving the compute on edge devices underutilized.

This motivates the study of \emph{edge-remote systems}, in which small LMs at the edge collaborate with frontier models in the cloud. Such systems could reduce cloud costs and unlock new asynchronous workflows (\textit{e.g.} bug finding) that run on idle compute resources. However, the cost-accuracy tradeoff induced by edge-remote collaboration is not well understood. 

The cost-accuracy tradeoff is governed by fundamental cost and quality asymmetries between small edge and frontier remote LMs. 

\begin{itemize}
    \item \emph{Capabilities}: There is a well-known quality gap between small and large LMs~\cite{kaplan2020scaling}. Often this gap is even larger on real-world tasks than benchmark results would suggest (see Section X). Looking forward, we expect the gap to persist despite rapid improvements across small and large models.

    \item \emph{Cost}: Since frontier models have 10-1000x more parameters than small models, they of course require more hardware, power and memory to run. But there are other differences too: batching requests affects the cost differently depending on whether we're at the edge or in the cloud. In the cloud, the server host can batch requests across concurrent users, so an individual user only obtains marginal savings by batching their requests. In contrast, at the edge, generating a batch of hundreds of samples in parallel is often no more costly than generating a single sample~\cite{leviathan2023fast}. 
\end{itemize}

The asymmetries above motivate us to focus on \emph{divide-and-conquer} strategies, where the remote model dispatches parallel tasks to worker models at the edge (see \Cref{fig:system}).
% 
% Given a \textit{task} to be performed over a large \textit{context} (\textit{e.g.} a codebase),
Given a \textit{task}  to be performed over a large \textit{context} (\textit{e.g.} a codebase), a divide-and-conquer edge-remote system proceeds in three (potentially looped) steps:
\begin{enumerate}
    \item \textbf{Decompose} The remote model writes code that decomposes the task and context into a long list of \textit{jobs}, all without actually pre-filling (\textit{i.e.} ``reading") the entire context.
    \item \textbf{Execute} The edge model then executes the jobs in parallel and sends a selection of the responses back to the remote model.
    \item \textbf{Aggregate} The remote model aggregates the outputs from the edge and finalizes the task output or loops back to the decompose step.
\end{enumerate}
% Given a \textit{task} to be performed over a large \textit{context} (\textit{e.g.} a codebase),  have the remote model first write code that decomposes the task and context into a list of \textit{jobs} which are sent to the edge. The edge model then executes the jobs in parallel before sending selected outputs back to the remote model for synthesis.
% 
Divide-and-conquer is a natural choice given the asymmetries discussed above. Critically, this strategy promises to significantly reduce remote costs, since none of the context is directly processed in the cloud. Furthermore, by decomposing the task into “bite-sized” jobs, it mitigates the gap in capabilities between remote and edge models. And finally, by delegating batches of parallel jobs to the edge, divide-and-conquer systems can achieve higher utilization of edge hardware, improving quality at little additional cost. 

% To reduce cloud costs, the raw input tokens will not be sent to the remote LM. The latter only interacts with a small edge LM with full access to the input. To offset the small LM's limited capabilities, the task is decomposed into ``bite-sized'' tasks and the input is decomposed into chunks. Benefiting from local parallelism, the edge model can efficiently execute subtasks on chunks of input. 

Despite the simplicity of the divide-and-conquer approach described above, the design and hyperparameter space of these kinds of edge-remote systems are poorly understood.
In this work, we perform an extensive analysis centered on three core design choices. Each design choice provides a different ``knobs'' that be turned to trade off cost and quality. 
\begin{enumerate}
  \item \textbf{Model choice} \textit{How does the choice of model at the edge and in the cloud affect cost and quality?} At the edge, we consider models ranging from 1B to 8B parameters from the Llama~\citep{dubey2024llama3} and Qwen families~\citep{bai2024qwen2.5}. In the cloud, we consider leading frontier models such as GPT 4o, Claude Sonnet 3.5, and Llama 3.3 70B. We show the effects of model pairs in \Cref{subsec:results-model}.
  \item \textbf{Sequential Communication Protocols.} \textit{Can multiple rounds of communication improve quality? At what cost?} We consider two strategies for improving the quality via multi-round of communication: (a) simple retrying and (b) full multi-turn edge-remote conversations. (See \Cref{subsec:results-communication})
  \item \textbf{Parallel Workloads at the Edge.} \textit{How should we structure parallel workloads at the edge to maximize performance and minimize cost?} \Cref{subsec:results-workloads}. We consider two strategies for controlling the degree of parallelism of jobs at the edge: (a) random sampling and (b) chunking and decomposition. \Cref{subsec:results-workloads}
\end{enumerate}

There are several important takeaways from our analysis that can inform research and development of edge-remote systems going forward. Across a three challenging benchmarks spanning financial~\cite{islam2023financebench}, medical ~\cite{adams2024longhealth}, and scientific reasoning ~\cite{dasigi2021dataset} we show that:
\begin{itemize}
  \item Optimized edge-remote systems can recover the performance of remote-only systems while sending only \yell{10\%} of the tokens to the remote model.
  \item We can navigate the cost-accuracy Pareto frontier using both sequential and parallel test-time compute strategies. 
    \begin{itemize}
        \item \textbf{Model choice.} The size of the edge model . On scientific reasoning (QASPER), accuracy improves from $38\%$ to $66\%$ when moving from a 1B to 8B parameter edge model. The 8B parameter figure is a 6 percentage point improvement over the baseline set by GPT-4o acting in isolation. However, 8B edge models are challenging to run on some edge hardware, especially when latency is a constraint.
        \item \textbf{Sequential.} By increasing the number of sequential rounds of communication, we can tradeoff of increased cost for improved quality. For example, on financial reasoning (FinanceBench) with 3B parameter edge models and GPT-4o in the cloud, we can improve accuracy from $53\%$ to $70\%$ by simply increasing the maximum number of communication rounds. However, this nearly doubles the number of tokens processed by the remote model.
        \item \textbf{Parallel.} By increasing the number of parallel jobs at the edge, we can also boost quality. We show that this increased parallelism is free at the edge due to batching and the IO-bound nature of LLM inference.  For example, on medical reasoning (LongHealth), by increasing the number of random samples, we can improve accuracy from \yell{$X\%$} to \yell{$Y\%$}. Critically, we show that this leads only to a \yell{$1.0z\times$} in edge latency, due to batching.
    \end{itemize}
  \item In Section \ref{subsec:results-communication}, we perform a fine-grained error analysis, showing how different types of tasks are more or less amenable to the different strategies described above. For example, \yell{TODO}. We also highlight several types of tasks where divide-and-conquer systems remain ineffective. This motivates future work in joint remote-edge training. 
  % \item TODO
\end{itemize}
% Most existing divide-and-conquer strategies rely on \emph{brittle, hand-crafted workflows} (CITE MAP REDUCE LM, DOCETL and others). Task decomposition is nontrivial and domain-specific. While previous work typically uses only large LMs, it is unclear which task decompositions are suitable for two assymetric LMs. We started by hand-crafting systems for finance, medical, and academic research domains. We found that significant tuning is required to match simple baselines such as directly generating with the remote model (with full access to context) or retrieval augmented generation.

% We then proceeded to ask whether remote LLMs can discover and generate appropriate task decomposition. This approach draws parallels to Domain-Specific Languages (DSLs), where software designers have traditionally struggled with decomposing tasks into manageable abstractions, and where LLMs are showing great promise. We investigate one prototype of a domain-agnostic edge-remote system, which we call \system with two core principles:
% \begin{itemize}
%     \item The remote model communicates with the edge model via code generation, motivated by the observation that some subtasks  (e.g. chunking long context) can be performed more reliably and efficiently with code (cite evaporate, chain of code).
%     \item \emph{Test-time scaling} is leveraged in two ways:
%     \begin{itemize}
%         \item \emph{Sampling}. The edge cost model encourages batching, which we use for test-time compute strategies (e.g. sampling/majority vote), to bolster the reliability of the small edge LM. 
%         \item \emph{Looping}. The remote and local model can have as many back-and-forth communication rounds as needed to confidently solve the task or abstain.
%     \end{itemize}
% \end{itemize}

% In experiments across domains, we first characterize which design choices are needed to match hand-crafted workflows. 
% With ablation studies, we then assess the implications of each of the above principles. We find that repeated sampling on edge, accompanied by step-by-step reasoning on remote, are necessary for success (made this up). While certain tasks require back-and-forth looping (\textit{e.g.} medical), others are not (finance).
% We investigate cost-accuracy tradeoffs across model sizes and historical generations for both the remote and local models. We find that systems with as small as a 3B edge model (NAME) can match the remote model performance with XX fewer tokens. Given historical data, we project that performance can be improved by XX on the same hardware each year. 

% To conclude, our contributions are as follows: 
% \begin{itemize}
%     \item We extensively investigate a new class of edge-remote collaborative systems, which we believe to be inevitable given trends in model and hardware development.
%     \item We propose the desiderata for such systems (Sec XX), involving communication efficiency, “intelligence ratios” between remote and edge models, and scaling properties.
%     \item We propose an autonomous a domain-general architecture coined \system, which reasons in code to dispatch tasks to edge LMs, and compare it to hand-crafted pipelines
%     \item We identify the core components of an edge-remote system and characterize how it behaves on different domains using different sizes and generations of LMs for both edge and remote
% \end{itemize}




==> sections/archive/introduction_jan_9_afternoon.tex <==
\section{Introduction}
\label{sec:intro}
Frontier, cloud-hosted Language Models (LMs) now excel at challenging reasoning tasks such as repository-level programming, as well as financial, legal, and medical decision-making. Solving such tasks often requires integrating information across millions of context tokens. However, performing long-context reasoning tasks is expensive: processing a standard million-token code repository with OpenAI’s o1 costs $>\$15$ per query. With many input tokens, the computational cost is dominated by the prefill-stage computation, where a cache of keys and values is formed for every input token. How can we reduce frontier-model cost while maintaining quality?

To reduce the number of tokens processed by cloud-hosted LLMs, practitioners rely primarily on retrieval-augmented generation (RAG), where only a subset of corpus documents that are deemed most similar to the query are passed in-context to an LM. Relevance is determined either through keyword look-ups~\cite{robertson_relevance_2009}, neural embedding search~\cite{karpukhin2020dense,lewis2020retrieval,lee2019latent}, or search~\cite{nakano2021webgpt}. Retrieval reduces prefill-stage computation by simply filtering out tokens, but still the LM still processes raw chunks of text from the corpus. 
% Other forms of context compression involve “memory” mechanisms, in which the LM stores only relevant information from a previous context and attends the memory store during subsequent generations. 
% Retrieval augmented generation is a powerful paradigm for reducing cost, but we find it often underperforms long-context frontier models with full-access to the context. 

New opportunities emerge with small LMs (\textit{e.g.} with 1-7B parameters) which are rapidly improving in quality and can be run on commodity edge hardware at reasonable throughput. For example, an \textcolor{red}{XX} model can be run on a phone at \textcolor{red}{XX} tokens per second. Today, these models play a limited role in challenging reasoning workloads. Motivated by the cost asymmetry between cheap edge LMs and expensive but more capable remote LMs, we study edge-remote collaborative systems, where a small LM with complete access to the context, and an ability to scale inference-time compute, collaborates with a remote frontier LM without direct access to the context. Put differently, the edge model provides a compressed, task-relevant view of the context to the remote model. 
% following the instructions and verification of the remote model. 
We explore the design choices of edge-remote systems and measure the tradeoff between cost and quality.

When prototyping edge-remote systems, we identified three practical challenges: 

\begin{itemize}
    \item \emph{Identifying effective communication protocols.} Language models are designed to interact with humans, not other models. It is not clear how should a remote model effectively request data, ask questions, and provide guidance to an edge model.
    \item \emph{Edge model can be unreliable.} Despite recent improvements, small LMs often hallucinate and make mistakes that a larger LMs would not, even in relatively simple tasks like summarization or information extraction. It is unclear which of their outputs can be trusted and which tasks can be safely delegated to them.
    \item \emph{Unconventional use case for frontier models.} The various stages of LM training prepare frontier models to reason with full raw contexts. Can they make do with fragments of processed information at varying levels of fidelity? What kinds of \emph{procedural knowledge} do they possess, enabling them to sketch solutions to problems without seeing the raw data?
\end{itemize}

We identify three key design decisions which address the challenges above and improve the cost-quality tradeoff:

\begin{itemize}
    \item We propose prompting strategies and workflows that result in effective edge model performance as well as informative and concrete instructions from the big LM. We also point to strategies that do not work.m
    \item We use repeated sampling to improve the reliability of the edge models, in line with recent results on scaling test-time compute. 
    \item We use summarization and extraction to improve the remote model’s visibility into local context do XXXX.
\end{itemize}

We apply the edge-remote system to a suite of legal, medical, and financial reasoning benchmarks, and characterize the tradeoff between accuracy and cost (the number of tokens processed by the frontier model). We ablate the performance of the model and show which stages are crucial to performance, and which benefit from scaling inference-time compute. We then compare our method to frontier models with full access to the context as well as SoTA RAG baselines. 

We find that edge-remote systems recover \textcolor{red}{XXX} of the remote-model performance while processing \textcolor{red}{XXX} fewer tokens. They also offer cost-accuracy tradeoffs favorable to RAG systems: when both methods processing a nearly identical number of tokens, edge-remote is up to \textcolor{red}{XXX} better than RAG. 


==> sections/archive/introduction_until_jan20.tex <==
\section{Introduction}
\label{sec:intro}

Today's frontier, cloud-hosted Language Models (LMs) are proficient at challenging reasoning tasks, including programming across repositories and making decisions in financial, legal, and medical domains. While these models offer powerful capabilities, accessing them remains expensive: processing a standard million-token code repository with OpenAI's o1 costs $>\$15$ per query. 

At the same time, edge devices contain a substantial amount of underutilized compute that could potentially assist with these workloads. Small LMs (\textit{e.g.} with 1-7B parameters) can now run on smartphones and laptops at reasonable throughput (Apple's OpenELM, PhoneLM,llama.cpp), \textit{e.g.} - an \textcolor{red}{XX} model can process \textcolor{red}{XX} tokens per second on a phone. Motivated by this cost asymmetry and the rapidly improving quality of small LMs' (CITE), we ask the question: how can we leverage edge compute resources to support cloud LMs in complex reasoning workflows and improve the cost-quality trade-off?

%Leveraging edge computing to reduce computational load is not a new concept. 
The prevailing approach for offloading computational demands from cloud LMs is retrieval-augmented generation (RAG). In RAG systems, only the most relevant subset of corpus documents is provided to the LM, with relevance determined via methods such as keyword lookups~\cite{robertson_relevance_2009}, neural embedding search~\cite{karpukhin2020dense,lewis2020retrieval,lee2019latent}, or web search~\cite{nakano2021webgpt}. By performing retrieval locally, RAG systems reduce cloud costs by \textit{minimizing} the context that needs to be processed by the cloud LM.

In this work, we take a step further and investigate other ways --- beyond retrieval -- that edge compute can be leveraged to compress the tokens processed by cloud LMs.
% while simultaneously enhancing output quality. 
We focus on edge-remote collaborative systems where smaller edge LMs, with full access to the context, collaborate with more capable remote models. 
In principle, the edge models can handle token-intensive tasks such as summarization and information extraction, while deferring to the remote models for planning, reasoning and verification.
% With full access to the context and the ability to scale inference-time compute (CITE), edge models can handle a significant portion of the processing, delivering compressed, task-specific representations to the cloud LM as needed.

% The challenge of reducing computational load on cloud LMs has primarily been addressed through retrieval-augmented generation (RAG). In RAG systems, only the most relevant subset of corpus documents is passed to the LM, with relevance determined through keyword lookups~\cite{robertson_relevance_2009}, neural embedding search~\cite{karpukhin2020dense,lewis2020retrieval,lee2019latent}, or web search~\cite{nakano2021webgpt}. Retrieval can be run locally and reduce cloud cost by merely filtering out tokens. 



% Here, we propose a broader investigation of edge-remote collaborative systems, where small edge LMs work in tandem with more capable remote models. Beyond retrieval, edge models can summarize, extract information, and execute components in a multi-step plan. The edge model, with complete access to the context and ability to scale inference-time compute (CITE), can provide compressed, task-relevant views to the remote model.

However, in practice, there are several challenges that arise when implementing edge-remote systems: 

\begin{itemize}
    \item \emph{Effective communication protocols.} LMs are designed to interact with humans, not other models. It is not clear how should a remote model effectively request data, ask questions, and provide guidance to an edge model.
    \item \emph{Unreliability of edge models.} Despite recent improvements, small LMs often hallucinate and make mistakes that larger LMs would not, even in relatively simple tasks like summarization or information extraction. It is unclear which of their outputs can be trusted and which tasks can be safely delegated to them.
    \item \emph{Unconventional use case for frontier models.} The various stages of LM training prepare frontier models to reason with full raw contexts. Can they make do with fragments of processed information at varying levels of fidelity? What kinds of \emph{procedural knowledge} do they possess, enabling them to sketch solutions to problems without seeing the raw data?
\end{itemize}

We identify three key design decisions which address the challenges above and improve the cost-quality tradeoff:

\begin{itemize}
    \item We propose a communication strategy in which the cloud LM interacts with the edge LLM in two primary roles: (1) providing guidance and (2) synthesizing returned information. This establishes a two-way communication channel where tasks are delegated to edge resources. The edge LLM processes these tasks and returns information to the cloud LM, which then synthesizes the new input and either delegates further tasks or provides a final response.  
    \item We use repeated sampling to improve the reliability of the edge models, in line with recent results on scaling test-time compute. 
    \item We use summarization and extraction to improve the cloud LM's visibility into local context. 
\end{itemize}

We apply the edge-remote system to a suite of legal, medical, and financial reasoning benchmarks, and characterize the tradeoff between accuracy and cost (the number of tokens processed by the frontier model). We ablate different components of our system and show which stages are crucial to performance, and which benefit from scaling inference-time compute. We then compare our method to frontier models with full access to the context as well as SoTA RAG baselines. 

We find that edge-remote systems recover \textcolor{red}{XXX} of the remote-model performance while processing \textcolor{red}{XXX} fewer tokens. They also offer cost-accuracy tradeoffs favorable to RAG systems: when both methods process a nearly identical number of tokens, edge-remote is up to \textcolor{red}{XXX} better than RAG.


==> sections/archive/m01d29_introduction.tex <==

% For many problems the question 

% Feedback 
% (1) make sure to run the minions protocol with edge-edge
% (2) give some prescriptive recommendation based on problem type for what design choices to use

\section{Introduction}
\label{sec:intro}
Today's cloud-hosted frontier Language Models (LMs) can program across repositories and make complex decisions in financial, legal, and medical domains. However, accessing these models is expensive: processing a standard million-token code repository with OpenAI's o1 API costs $>\$15$ per query. 
% 
At the same time, smaller LMs (1-8B parameters) are rapidly improving and can now run on personal computers (ollama, llama.cpp) and smartphones (OpenELM, PhoneLM)  (\textit{e.g.} an \textcolor{red}{XX} model can process \textcolor{red}{XX} tokens per second on a phone). 
%
Currently, small edge LMs are used exclusively for simple tasks such as text completion and summarization, while advanced reasoning tasks are typically handled entirely in the cloud by frontier models. 


% How can we do more on edge? And what does this mean or the cost / acc of frontier models/
We ask: \textit{how can we utilize a small LM on-device to reduce cloud inference costs}? Our setting includes two models interacting in natural language: a frontier LM in the cloud (\textit{e.g.} \textit{\gpt}) and a small LM running on-device with exclusive access to context (\textit{e.g.} \llama-3B). See \cref{sec:prelim-setting} for a detailed description of the setting under study.

We draw inspiration from real-world workflows and focus on tasks that require reasoning over large volumes of financial, medical, and scientific text. The text, such as a company's 10-K financial statement, is assumed to be stored locally. The user specifies a task that can range from simple information extraction (``What was the total revenue in FY2023?'') to multi-step calculations (\yell{Sabri, can you copy a concrete example of a calculation}?).

% Inspired by recent work on multi-agent systems (CITE MoA), 
% we study an asymmetric collaboration setting where a small edge LM (\textit{e.g.} Llama-2-3.2B), with full access to the input, communicates with a frontier cloud-hosted LM (\textit{e.g.} Claude-Sonnet-3.5) without access to the input.

We first consider a basic turn-taking communication protocol (\naive), that is, a chat between the local and remote model. By having only the local model ``read'' the full context, we can achieve a $\yell{20}\times$ reduction in remote model costs, however, losing  \yell{10\%}  (see \Cref{sec:naive} for details)
% (
However, this naïve protocol struggles to recover the performance of the frontier model. 

% We identify two reasons why the \naive protocol is suboptimal for the edge-remote setting:

% Need to make this very concrete with a forward pointer to exact definition of what this naive sysytem looks like 
% Below, I think we can drop the middle bullet and these should also just point to a section where we highlight the limitations of the naive back and forth.

\begin{itemize}
    \item  \emph{Limitations of small LMs.} The well-known quality gap between large and small models \cite{kaplan2020scaling} is even more pronounced on the real-world workflows under study. We find two core limitations that hamper an unconstrained back-and-forth chat:
    \begin{itemize}
        \item \textbf{Long-context processing}. Small LMs can get distracted and incoherent when processing long sequences of tokens.
        \item \textbf{Multi-step instruction following} Small LMs cannot be trusted to follow multi-step instructions.
    \end{itemize}
    
    Small models struggle with long contexts and do not adhere to the complex, multi-part instructions output by large models. We explore these limitations in \Cref{sec:naive-quality}.
    % \item Frontier LM's need to \emph{calibrate} to the capabilities of the small LMs and infer when can their outputs be trusted.
    \item \emph{Low utilization of on-device resources.} As we discuss in \Cref{sec:naive-util}, this protocol achieves only \yell{X\%} hardware utilization at the edge because LM inference is I/O bound with batch size one. In the cloud, this isn't a problem because the server host can batch requests across concurrent users. However, at the edge, generating a hundred samples in parallel is often no more costly than generating a single sample \cite{leviathan2023fast}.  Therefore, this sequential turn-taking protocol leaves significant edge compute on the table.
\end{itemize}

% Needs forward pointer to exact method defintiion and pointer to figure showing the method
Motivated by these limitations, we propose a simple extension of this protocol, coined \system  (emphasis on the $\mathcal{S}$), where the remote model decomposes the task into \emph{subtasks} that can be executed \emph{in parallel} on device. 

But how can the remote model perform a fine-grained task decomposition \emph{without seeing any data}? Our first obseration is that given a question, a frontier model possess an impressive amount of ``procedural knowledge'', \textit{i.e.} which steps are needed to answer a question, and which data each requires.

A second problem, is that not only we need to decompose the task: the context needs to be chunked at some chosen level of granularity, and passed to the local model along with a subtask.  To achieve that, our second insight is to generate code by the remote model, that can be executed locally where context is available, to flexibly chunk the document and assign tasks to individual chunks.

% 
\system has three steps, which are performed in a loop:
\begin{enumerate}
    \item \textbf{Decompose} Given a task, the remote model writes code that decomposes the task and context into a long list of ``bite-sized'' \textit{subtasks}.
    \item \textbf{Execute} The edge model then executes the subtasks in parallel and sends a filtered selection of the responses back to the remote model.
    \item \textbf{Aggregate} The remote model aggregates the outputs from the edge and finalizes the task output or loops back to the Decompose step.
\end{enumerate}

% This protocol is motivated by a rich literature, ~\cite{mixtur} \yell{the sequential nature should be explained, they may ask about what can or cannot be broken down in this way}.
\system is a natural choice given the challenges discussed above. By decomposing the task into “bite-sized” jobs, it mitigates the gap in capabilities between remote and edge models. And finally, by delegating batches of parallel jobs to the edge, \system can achieve higher utilization of edge hardware, improving quality at little additional cost. 


% Can probably drop first sentence
% To reiterate, all remote computations are done without pre-filling (\textit{i.e.} ``reading") the entire input. In fact, we find that by communicating less than 10\% of the total input tokens to the cloud, MINION performs comparably to the frontier model in finance, health, and academic paper QA benchmarks \yell{CITE}. 

% MINION is a natural choice given the asymmetries discussed above. Critically, this strategy promises to significantly reduce remote costs, since none of the context is directly processed in the cloud. Furthermore, by decomposing the task into “bite-sized” jobs, it mitigates the gap in capabilities between remote and edge models. And finally, by delegating batches of parallel jobs to the edge, divide-and-conquer systems can achieve higher utilization of edge hardware, improving quality at little additional cost. 

% We identify three key design choices (i.e. hyperparameters) that govern this protocol. However, it is unlear how they affect the cost-accuracy tradeoff. We analyze this:

Despite the intuitive appeal of such edge-remote communication protocols, we have a poor understanding of their design and hyperparameter space which in turn serve as ``knobs'' that trade off cost for quality. Concretely:
\begin{enumerate}
  \item \textbf{Model choice} \textit{How does the choice of model at the edge and in the cloud affect cost and quality?} At the edge, we consider models ranging from 1B to 8B parameters from the \llama~\citep{dubey2024llama3} and \qwen families~\citep{bai2024qwen2.5}. In the cloud, we consider leading frontier models such as \gpt, Claude Sonnet 3.5, and \llama-3.3-70B. We show the effects of model pairs in \Cref{subsec:results-model}.
  \item \textbf{Sequential Communication Protocols.} \textit{Can multiple rounds of communication improve quality? At what cost?} We consider two strategies for improving the quality, through looping of the \system steps (a)``retry'': increasing the number of attempts for the \system system, where each attempt is blind to previous attempts (b) allowing longer multi-turn conversations where the remote model sees the results of the previous attempts (See \Cref{subsec:results-communication})
  \item \textbf{Parallel Workloads at the Edge.} \textit{How should we structure parallel workloads at the edge to maximize performance and minimize cost?} \Cref{subsec:results-workloads}. We consider two strategies for controlling the degree of parallelism of jobs at the edge: (a)  repeated sampling~\citep{brown2024large} and (b) chunking and decomposition. \Cref{subsec:results-workloads}
\end{enumerate}

In Section \ref{subsec:results-communication}, we perform an error analysis, showing how different types of tasks are more or less amenable to the different strategies described above. For example, \yell{TODO}. We also highlight several types of tasks where divide-and-conquer systems remain ineffective. This motivates future work in joint remote-edge training.


There are several important takeaways from our analysis that can inform research and development of edge-remote systems going forward. Across a three challenging benchmarks spanning financial~\cite{islam2023financebench}, medical ~\cite{adams2024longhealth}, and scientific reasoning ~\cite{dasigi2021dataset} we show that \yell{add short description on task hierarchies and why we chose these}:
\begin{itemize}
  \item Optimized edge-remote systems can recover the performance of remote-only systems while sending only \yell{10\%} of the tokens to the remote model.
  \item We can navigate the cost-accuracy Pareto frontier using both sequential and parallel test-time compute strategies. 
    \begin{itemize}
        \item \textbf{Model choice.} The size of the edge model . On scientific reasoning (\qasper), accuracy improves from $38\%$ to $66\%$ when moving from a 1B to 8B parameter edge model. The 8B parameter figure is a 6 percentage point improvement over the baseline set by GPT-4o acting in isolation. However, 8B edge models are challenging to run on some edge hardware, especially when latency is a constraint.
        \item \textbf{Sequential.} By increasing the number of sequential rounds of communication, we can tradeoff of increased cost for improved quality. For example, on financial reasoning (\finance) with 3B parameter edge models and GPT-4o in the cloud, we can improve accuracy from $53\%$ to $70\%$ by simply increasing the maximum number of communication rounds. However, this nearly doubles the number of tokens processed by the remote model.
        \item \textbf{Parallel.} By increasing the number of parallel jobs at the edge, we can also boost quality. We show that this increased parallelism is free at the edge due to batching and the IO-bound nature of LLM inference.  For example, on medical reasoning (\longhealth), by increasing the number of random samples, we can improve accuracy from \yell{$X\%$} to \yell{$Y\%$}. Critically, we show that this leads only to a \yell{$1.0z\times$} in edge latency, due to batching.
    \end{itemize}
  \item In Section \ref{subsec:results-communication}, we perform a fine-grained error analysis, showing how different types of tasks are more or less amenable to the different strategies described above. For example, \yell{TODO}. We also highlight several types of tasks where divide-and-conquer systems remain ineffective. This motivates future work in joint remote-edge training. 
\end{itemize}




==> sections/archive/m09d20introduction.tex <==
\section{Introduction}
\label{sec:intro}
Today's frontier Language Models (LMs) are proficient at challenging reasoning tasks, including programming across repositories and making decisions in financial, legal, and medical domains. Accessing the most capable models on the cloud remains expensive: processing a standard million-token code repository with OpenAI's o1 costs $>\$15$ per query. 

At the same time, edge devices contain a substantial amount of underutilized compute that could potentially assist with these workloads. Smaller LMs (\textit{e.g.} with 1-70B parameters) are rapidly improving and can now be run on personal computers (ollama, llama.cpp) and smartphones (OpenELM, PhoneLM) at low latency - \textit{e.g.} - an \textcolor{red}{XX} model can process \textcolor{red}{XX} tokens per second on a phone. Currently, small LMs are not participating in challenging reasoning tasks. 

Here, we ask to which extent can small LMs on device can collaborate with frontier models on the cloud. Such \emph{edge-remote systems} can reduce cloud costs and unlock new asynchronous workflows (e.g. bug finding) that run on idle compute resources. By offloading computation to cheaper but less capable LMs, we introduce a cost-accuracy tradeoff which we explore in this work.

The tradeoff is governed by three fundamental asymmetries between edge and remote LMs. 

\begin{itemize}
    \item \emph{Capabilities}: The well-known gap between small and large LMs is even larger on real-world tasks than benchmark results would suggest (see Section X). We expect the gap to persist despite rapid improvements across small and large models.
    
    \item \emph{Cost (in \$)}: Edge processing is free. Remote processing is \$.

    \item \emph{Runtime savings from parallelism}: In LLM inference, generating a batch of samples in parallel is often no more costly than generating a single sample. This is because when batch sizes are small, LLM inference is I/O bound. The inference server host controls batching and can thus save costs by batching requests across concurrent users, as typically done by model providers. Users can only obtain marginal savings by sending a batch of requests. In contrast, a locally running inference server, on the other hand, implies that users incur a latency cost when processing less than full batches of requests.
\end{itemize}

The assymetries above motivate the following \emph{divide-and-conquer} strategy. To reduce cloud costs, the raw input tokens will not be sent to the remote LM. The latter only interacts with a small edge LM with full access to the input. To offset the small LM's limited capabilities, the task is decomposed into ``bite-sized'' tasks and the input is decomposed into chunks. Benefiting from local parallelism, the edge model can efficiently execute subtasks on chunks of input. 

Most existing divide-and-conquer strategies rely on \emph{brittle, hand-crafted workflows} (CITE MAP REDUCE LM, DOCETL and others). Task decomposition is nontrivial and domain-specific. While previous work typically uses only large LMs, it is unclear which task decompositions are suitable for two assymetric LMs. We started by hand-crafting systems for finance, medical, and academic research domains. We found that significant tuning is required to match simple baselines such as directly generating with the remote model (with full access to context) or retrieval augmented generation.

We then proceeded to ask whether remote LLMs can discover and generate appropriate task decomposition. This approach draws parallels to Domain-Specific Languages (DSLs), where software designers have traditionally struggled with decomposing tasks into manageable abstractions, and where LLMs are showing great promise. We investigate one prototype of a domain-agnostic edge-remote system, which we call \textbf{MINION} with two core principles:
\begin{itemize}
    \item The remote model communicates with the edge model via code generation, motivated by the observation that some subtasks  (e.g. chunking long context) can be performed more reliably and efficiently with code (cite evaporate, chain of code).
    \item \emph{Test-time scaling} is leveraged in two ways:
    \begin{itemize}
        \item \emph{Sampling}. The edge cost model encourages batching, which we use for test-time compute strategies (e.g. sampling/majority vote), to bolster the reliability of the small edge LM. 
        \item \emph{Looping}. The remote and local model can have as many back-and-forth communication rounds as needed to confidently solve the task or abstain.
    \end{itemize}
\end{itemize}

In experiments across domains, we first characterize which design choices are needed to match hand-crafted workflows. 
With ablation studies, we then assess the implications of each of the above principles. We find that repeated sampling on edge, accompanied by step-by-step reasoning on remote, are necessary for success (made this up). While certain tasks require back-and-forth looping (\textit{e.g.} medical), others are not (finance).
We investigate cost-accuracy tradeoffs across model sizes and historical generations for both the remote and local models. We find that systems with as small as a 3B edge model (NAME) can match the remote model performance with XX fewer tokens. Given historical data, we project that performance can be improved by XX on the same hardware each year. 

To conclude, our contributions are as follows: 
\begin{itemize}
    \item We extensively investigate a new class of edge-remote collaborative systems, which we believe to be inevitable given trends in model and hardware development.
    \item We propose the desiderata for such systems (Sec XX), involving communication efficiency, “intelligence ratios” between remote and edge models, and scaling properties.
    \item We propose an autonomous a domain-general architecture coined MINION, which reasons in code to dispatch tasks to edge LMs, and compare it to hand-crafted pipelines
    \item We identify the core components of an edge-remote system and characterize how it behaves on different domains using different sizes and generations of LMs for both edge and remote
\end{itemize}


==> sections/impact_statement.tex <==
\section*{Impact Statement}
\system advances cost-efficient AI by demonstrating how small on-device language models can collaborate with powerful cloud-hosted models to perform data-intensive reasoning. By reducing reliance on expensive remote inference, \system makes advanced AI more accessible and sustainable. This has broad societal implications, including lowering barriers to AI adoption and enhancing data privacy by keeping more computations local. However, careful consideration must be given to potential biases in small models and the security risks of local code execution. 

==> tables/long_context_results.tex <==
\begin{table}[ht]
    \centering
    \scriptsize
\begin{tabular}{llllllllllll}
                                                & \multicolumn{3}{c}{\textbf{Model}}                     & \multicolumn{2}{c}{\textbf{FinanceBench}} & \multicolumn{2}{c}{\textbf{LongHealth}} & \multicolumn{2}{c}{\textbf{QASPER}} & \multicolumn{2}{c}{\textbf{RepoQA}} \\
                                                & Edge          & Remote            & Retrieval & Accuracy  & Cost & Accuracy         & Cost        & Accuracy       & Cost      & Accuracy       & Cost      \\ \hline \hline
\textbf{Remote Only }                         & ---           & GPT-4o            & ---       &           &                      &                  &             &                &           &                &           \\
                                                & ---           & Llama-3.3-70b     & ---       &           &                      &                  &             &                &           &                &           \\
                                                & ---           & Claude 3.5 Sonnet & ---       &           &                      &                  &             &                &           &                &           \\
\textbf{Edge Only }                           & Llama-3.2-3b  & ---               & ---       &           &                      &                  &             &                &           &                &           \\
                                                & LLlama-3.2-1b & ---               & ---       &           &                      &                  &             &                &           &                &           \\
\textbf{Remote + Retrieval }             & ---           & GPT-4o            & BM25      &           &                      &                  &             &                &           &                &           \\
                                                & ---           & GPT-4o            & OpenAI    &           &                      &                  &             &                &           &                &           \\ \hline
\textbf{Remote + Edge  }            & Llama-3.2-3b  & GPT-4o            & ---       &           &                      &                  &             &                &           &                &           \\
                                                & Llama-3.2-3b  & Llama-3.3-70b     & ---       &           &                      &                  &             &                &           &                &           \\
                                                & Llama-3.2-3b  & Claude 3.5 Sonnet & ---       &           &                      &                  &             &                &           &                &           \\
\textbf{Remote + Edge + Retrieval} & Llama-3.2-3b  & GPT-4o            & BM25      &           &                      &                  &             &                &           &                &           \\
                                                & Llama-3.2-3b  & Llama-3.3-70b     & BM25      &           &                      &                  &             &                &           &                &           \\ \hline
\end{tabular}
\caption{\textbf{Evaluation on long-context benchmarks.}}
\end{table}
